Reconstructing a graph from its Bell colouring graph

The Bell colouring graph $\mathcal{B}(G)$ of a graph $G$ is the graph whose vertices are the partitions of the vertex set of $G$ into independent sets, with an edge between two partitions if and only if one can be obtained from the other by changing the part of a single vertex of $G$. Given a natural number $k$, the Bell $k$-colouring graph $\mathcal{B}_k(G)$ and the upper-Bell $k$-colouring graph $\mathcal{B}_{\geq k}(G)$ are the induced subgraphs of $\mathcal{B}(G)$ consisting of all partitions with at most $k$ parts and at least $k$ parts, respectively. We determine precisely when two finite graphs have isomorphic Bell colouring graphs. In particular, we show that every $n$-vertex graph $G$ with no vertices of degree $n-1$ is uniquely determined by its Bell colouring graph $\mathcal{B}(G)$, and by its upper-Bell colouring graph $\mathcal{B}_{\geq k}(G)$ if $k\leq n-2$. We also show that every $n$-vertex graph with maximum degree $\Delta(G)< \frac{1}{9}n-\frac{1}{3}$ is uniquely determined by its Bell $k$-colouring graph $\mathcal{B}_k(G)$ if $k>\chi(G)$. By taking graph complements, each of these results can be restated in terms of partitions into cliques.

==> tikzcommands.tex <==
\RequirePackage{xparse} % ensures \NewDocumentCommand is available

\NewDocumentCommand{\drawcircle}{ O{0.4} m }{%
  % #1 = optional radius (default 0.4)
  % #2 = coordinate name (without parentheses)
  \draw[blue!70!black, line width=0.8pt, fill=blue!10] (#2) circle (#1);
  \node[dot] at (#2) {};
}

\NewDocumentCommand{\drawlabelledcircle}{ O{0.4} m m }{%
  % #1 = optional radius (default 0.4)
  % #2 = coordinate name (without parentheses)
  % #3 = label text
  \draw[blue!70!black, line width=0.8pt, fill=blue!10] (#2) circle (#1);
  \node[] at (#2) {$#3$};
}

\newcommand{\drawcapsule}[3]{%
  % #1 = first coordinate name, #2 = second coordinate name
  % midpoint, #2 = expand factor
  \coordinate (M) at ($0.5*(#1)+0.5*(#2)$);
  \def\expandfactor{#3}
  % expanded endpoints
  \coordinate (Aout) at ($(M)! \expandfactor ! (#1)$);
  \coordinate (Bout) at ($(M)! \expandfactor ! (#2)$);
  % draw capsule
  \draw[line cap=round, line width=0.8pt,
        draw=blue!70!black, double=blue!10,
        double distance=16*\expandfactor] (Aout) -- (Bout);
  % draw the dots
  \node[dot] at (#1) {};
  \node[dot] at (#2) {};
}

\newcommand{\drawlabelledcapsule}[5]{%
  % #1 = first coordinate name, #2 = second coordinate name
  % midpoint
  \coordinate (M) at ($0.5*(#1)+0.5*(#2)$);
  \def\expandfactor{#5}
  % expanded endpoints
  \coordinate (Aout) at ($(M)! \expandfactor ! (#1)$);
  \coordinate (Bout) at ($(M)! \expandfactor ! (#2)$);
  % draw capsule
  \draw[line cap=round, line width=0.8pt,
        draw=blue!70!black, double=blue!10,
        double distance=12*\expandfactor] (Aout) -- (Bout);
  % draw the dots
  \node[] at (#1) {$#3$};
  \node[] at (#2) {$#4$};
}

\newcommand{\drawroundedtriangle}[4][2]{%
  % #1 = expansion factor (default 2)
  % #2, #3, #4 = coordinate names of the triangle vertices (no parentheses)  
  % centroid
  \coordinate (G) at ($1/3*(#2) + 1/3*(#3) + 1/3*(#4)$);
  % expanded vertices (for the rounded triangle)
  \coordinate (Aout) at ($(G)!#1!(#2)$);
  \coordinate (Bout) at ($(G)!#1!(#3)$);
  \coordinate (Cout) at ($(G)!#1!(#4)$);
  % draw the rounded triangle
  \draw[rounded corners=11pt, line width=1pt, fill=blue!10, draw=blue!70!black]
    (Aout) -- (Bout) -- (Cout) -- cycle;
  % draw the dots
  \node[dot] at (#2) {};
  \node[dot] at (#3) {};
  \node[dot] at (#4) {};
}

\newcommand{\drawlabelledroundedtriangle}[7][2]{%
  % #1 = expansion factor (default 2)
  % #2, #3, #4 = coordinate names of the triangle vertices (no parentheses)
  % centroid
  \coordinate (G) at ($1/3*(#2) + 1/3*(#3) + 1/3*(#4)$);
  % expanded vertices (for the rounded triangle)
  \coordinate (Aout) at ($(G)!#1!(#2)$);
  \coordinate (Bout) at ($(G)!#1!(#3)$);
  \coordinate (Cout) at ($(G)!#1!(#4)$);
  % draw the rounded triangle
  \draw[rounded corners=11pt, line width=1pt, fill=blue!10, draw=blue!70!black]
    (Aout) -- (Bout) -- (Cout) -- cycle;
  % draw the dots
  \node[] at (#2) {$#5$};
  \node[] at (#3) {$#6$};
  \node[] at (#4) {$#7$};
}

\makeatletter
% key defaults for the bent-oval macro
\pgfkeys{
  /bentoval/.is family, /bentoval,
  radius/.initial = 2.0,
  width/.initial  = 0.6,
  fill/.initial   = blue!10,
  draw/.initial   = blue!60
}

\newcommand{\bentoval}[4][]{%
  % apply keys
  \pgfkeys{/bentoval, #1}%
  % create temporary coordinates
  \coordinate (BV@O) at #2;
  \coordinate (BV@A) at #3;
  \coordinate (BV@B) at #4;
  % get cartesian coords (in pt)
  \path (BV@A); \pgfgetlastxy{\BV@Ax}{\BV@Ay};
  \path (BV@B); \pgfgetlastxy{\BV@Bx}{\BV@By};
  \path (BV@O); \pgfgetlastxy{\BV@Ox}{\BV@Oy};
  % differences
  \pgfmathsetmacro{\BV@dxA}{\BV@Ax-\BV@Ox}%
  \pgfmathsetmacro{\BV@dyA}{\BV@Ay-\BV@Oy}%
  \pgfmathsetmacro{\BV@dxB}{\BV@Bx-\BV@Ox}%
  \pgfmathsetmacro{\BV@dyB}{\BV@By-\BV@Oy}%
  % angles (degrees)
  \pgfmathsetmacro{\BV@angA}{atan2(\BV@dyA,\BV@dxA)}%
  \pgfmathsetmacro{\BV@angB}{atan2(\BV@dyB,\BV@dxB)}%
  % normalize so arc goes the short/expected way
  \pgfmathsetmacro{\BV@angBnorm}{ifthenelse(\BV@angB<\BV@angA, \BV@angB+360, \BV@angB)}%
  % key values
  \pgfkeysgetvalue{/bentoval/radius}{\BV@radius}%
  \pgfkeysgetvalue{/bentoval/width}{\BV@width}%
  \pgfkeysgetvalue{/bentoval/fill}{\BV@fill}%
  \pgfkeysgetvalue{/bentoval/draw}{\BV@draw}%
  % define points on inner/outer radii
  \path (BV@O) ++(\BV@angA:\BV@radius) coordinate (BV@Pinner);
  \path (BV@O) ++(\BV@angBnorm:\BV@radius) coordinate (BV@Qinner);
  \path (BV@O) ++(\BV@angBnorm:{\BV@radius+\BV@width}) coordinate (BV@Qouter);
  \path (BV@O) ++(\BV@angA:{\BV@radius+\BV@width}) coordinate (BV@Pouter);
  % draw the bent oval (filled)
  % Note: connect tangents use the input-point angles (BV@angBnorm and BV@angA)
  \fill[\BV@fill, draw=\BV@draw, very thick]
    (BV@Pinner) arc (\BV@angA:\BV@angBnorm:\BV@radius)
    to[out=\BV@angBnorm+90,in=\BV@angBnorm+90] (BV@Qouter)
    arc (\BV@angBnorm:\BV@angA:{\BV@radius+\BV@width})
    to[out=\BV@angA-90,in=\BV@angA-90] (BV@Pinner);
}
\makeatother

\newcommand{\doublecurve}{
\tikz[baseline={(0,-0.2)}]{
  \draw[bend left=60]  (0,0) to (0.15,0);
  \draw[bend right=60] (0,0) to (0.15,0);
  \fill (0,0) circle (0.9pt);
  \fill (0.15,0) circle (0.9pt);
}}

\newcommand{\supclaw}{
\tikz[scale=0.8,baseline={(0,-0.08)}]{
  \draw (0,0) to (0.15,0.06);
  \draw (0,0) to (0.15,0);
  \draw (0,0) to (0.15,-0.06);
  \fill (0,0) circle (0.6pt);
  \fill (0.15,0.06) circle (0.6pt);
  \fill (0.15,0) circle (0.6pt);
  \fill (0.15,-0.06) circle (0.6pt);
}}

\newcommand{\claw}{
\tikz[scale=0.8,baseline={(0,-0.12)}]{
  \draw (0,0) to (0.15,0.06);
  \draw (0,0) to (0.15,0);
  \draw (0,0) to (0.15,-0.06);
  \fill (0,0) circle (0.6pt);
  \fill (0.15,0.06) circle (0.6pt);
  \fill (0.15,0) circle (0.6pt);
  \fill (0.15,-0.06) circle (0.6pt);
}}
